On Hierarchical Communication Topologies in the pi-calculus

This paper is concerned with the shape invariants satisfied by the communication topology of {\pi}-terms, and the automatic inference of these invariants. A {\pi}-term P is hierarchical if there is a finite forest T such that the communication topology of every term reachable from P satisfies a T-shaped invariant. We design a static analysis to prove a term hierarchical by means of a novel type system that enjoys decidable inference. The soundness proof of the type system employs a non-standard view of {\pi}-calculus reactions. The coverability problem for hierarchical terms is decidable. This is proved by showing that every hierarchical term is depth-bounded, an undecidable property known in the literature. We thus obtain an expressive static fragment of the {\pi}-calculus with decidable safety verification problems.

==> definitions/bisimA.tex <==
Let $Q$ be a term reachable from $P$ and
$(\qready, f)$ be a configuration of an automaton $\Aut$.
Let $\phi = \Phi'(Q)$,
the relation $Q \bisimA f$ holds if and only if
there exists an injective function $\iota \from \nodes(\phi) \to \dataset$
such that for all $n \in \nodes(\phi)$:
\begin{enumerate}[label=\roman*)]
  \item if $\iota(n) = d$, $n' \parent_\phi n$ and $\iota(n') = d'$ then
        $d' = \pred(d)$;
  \item if $n$ is labelled with $(\chi_i, t)$ then $f(\iota(n)) = \chi_i$;
  \item if $n$ is labelled with a sequential process $Q'$ then
        $f(\iota(n)) = Q'$;
  \item for each $d$ such that $f(d) \neq \fresh$ either
          there is an $n$ such that $\iota(n) = d$
            or
          $f(d) = \qdead$.
\end{enumerate}

==> definitions/phi.tex <==
\begin{equation*}
  \Phi_\Types(\new X.\Parallel_{i \in I} A_i) \is
    \begin{cases}
      \Dunion_{i\in I} \set{A_i[]} \CASE X = \emptyset \\
        \left(
          \Dunion
            \set{(x,\base(\type))[ \Phi_\Types(\new Y_x.\Parallel_{j \in I_x} A_j) ]
                | (x\tas\type) \in \minrestr(X) }
          % \Dunion_{(x\tas\type) \in \minrestr(X)}
          %   (x,\base(\type))[ \Phi(\new Y_x.\Parallel_{j \in I_x} A_j) ]
        \right)
      \dunion
      \Phi_\Types(\new Z.\Parallel_{r\in R} A_r)
      \CASE X \neq \emptyset
    \end{cases}
\end{equation*}
where
\ifshortversion%
  $P = \new X.\Parallel_{i \in I} A_i$,
  $I_x = \set{i\in I | x \ntiedto{P} i}$,
  $R = I \setminus (\Union_{(x\tas\type) \in \minrestr(X)} I_x)$,
  $Y_x = \set{(y \tas \type) \in X | \exists i \in I_x \, .\, y \in \freenames(A_i)} \setminus \minrestr(X)$ and
  $Z = X \setminus (\Union_{(x\tas\type) \in \minrestr(X)} Y_x \union \set{x \tas \type})$.
\else%
    $P = \new X.\Parallel_{i \in I} A_i$ and
  \begin{align*}
    I_x &= \set{i\in I | x \ntiedto{P} i} &
    R &= I \setminus (\textstyle \Union_{(x\tas\type) \in \minrestr(X)} I_x)\\
    Y_x &= \set{(y \tas \type) \in X | \exists i \in I_x \, .\, y \in \freenames(A_i)} \setminus \minrestr(X) &
    Z &= X \setminus (\textstyle \Union_{(x\tas\type) \in \minrestr(X)} Y_x \union \set{x \tas \type})
  \end{align*}
\fi%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $Y_x = \set{(y\tas\type) \in X | y \in \freenames(A_i), y \neq x, i \in I_x}$,
% $R = \set{i\in I | \nexists x \in \minrestr(X) \st x \ntiedto{P} i}$ and
% $Z = \set{(z\tas\type) \in X | z \not\in \minrestr(X), \forall x \in \minrestr(X) \st z \not\in Y_x}$.\\

==> definitions/react.tex <==
We define for each $D \in \Deriv$ the set of transition expressions
$\trgen{React}(D)$ representing the steps needed to simulate in the automaton
the potential reactions of $D$.
\begin{align*}
  \trgen{React}(M) &\is \trgen{React}_{\qdead}^M(M) \\
  \trgen{React}(\bang{M}) &\is \trgen{React}_{\bang{M}}^{\bang{M}}(M)
\end{align*}
The set of transition expressions $\trgen{React}_q^D(M)$ collects all the
potential reactions of $M$ as a choice of $D$;
the label $q$ is the one that should be associated with
the ``consumed'' term $D$ after a reaction has been completed.
The transitions simulating a replicated component will not mark,
as the ones for non replicated terms, the reacted term with $\qdead$,
which will represent ``garbage'' inert nodes in $f$.
The term $\zero$ cannot initiate any step and a choice may do any action
that one of its choices can:
\begin{align*}
  \trgen{React}_q^D(\zero) &\is \emptyset \\
  \trgen{React}_q^D(M+M') &\is \trgen{React}_q^D(M) \union \trgen{React}_q^D(M')
\end{align*}
Any sender can initiate a synchronisation from the ready state:
\bgroup
\newcommand{\nudge}{\\&\hspace{-7.5em}} %% Horrible spacing hack
\begin{align*}
  \trgen{React}_q^D(\out \chi_t<\chi_{t'}>.C) \is
    \nudge
    \set{\enctr{\qready,  \chi_t \chi_{t'} D}
               {q', \s{\chi_t}{syn} \s{\chi_{t'}}{msg} \s{C}{wait}}
      | t < t'}
    \nudge\union
    \set{\enctr{\qready,  \chi_{t'} \chi_t D}
               {q', \s{\chi_{t'}}{msg} \s{\chi_t}{syn} \s{C}{wait}}
      | t > t'}
    \nudge\union
    \trgen{Spawn}(q', \q{send}, \s{C}{wait}, q, \Phi'(C)).
\end{align*}
\egroup
where $q'$ is fresh.
Here, the state $\q{send}$ signals that we are in the middle of a synchronisation,
where the sender is committed but a receiver has yet to be selected.

For the case of an input prefix $M = \inp\chi_t(x).C$ we distinguish two cases:
when the base type of $\chi_t$ is greater than the base type of $x$
no migration occurs, otherwise part of the continuation needs to be spawned
in the sender's path.
In the case when the base type of $\chi_t$ is greater than the base type of $x$,
we set
\bgroup
\newcommand{\nudge}{\\&\hspace{-7.5em}} %% Horrible spacing hack
\begin{align*}
  \trgen{React}_q^D(\inp\chi_t(x).C) \is
    \nudge
    \set{\enctr{\q{send}, \s{\chi_t}{syn} \s{\chi_{t'}}{msg} D}
               {\q{rec},  \chi_t \chi_{t'} \s{C}{rec}}
        | t \tlt t' \in \Types}
    \nudge
    \set{\enctr{\q{send}, \s{\chi_{t'}}{msg} \s{\chi_t}{syn} D}
               {\q{rec},  \chi_{t'} \chi_t \s{C}{rec}}
        | t > t' \in \Types}
    \nudge\union
    \trgen{Spawn}(\q{rec}, \qready, \s{C}{rec}, q, \Phi'(C)).
\end{align*}
\egroup
In the case when the base type of $\chi_t$ is greater than the base type of $x$,
more transitions are required.
First, we precompute for each $M = \inp\chi_t(x).C$ as above
and $t \tlt t' \in \Types$,
the two forests $\mig{C, t'}$ and $\nmig{C}$ such that
$\Phi'(C\subst{x -> \chi_{t'}}) = \mig{C, t'} \dunion \nmig{C}$ and
$\mig{C, t'}$ contains all the nodes labelled with sequential terms
tied to $\chi_{t'}$ in $C\subst{x -> \chi_{t'}}$.
As we have shown in the proof of Theorem~\ref{th:typed-tshaped},
by virtue of Lemma~\ref{lemma:tied-tree},
$\mig{C, t'}$ and $\nmig{C}$ are indeed disjoint.
Then we set:
\bgroup
\newcommand{\nudge}{\\&\hspace{-7.5em}} %% Horrible spacing hack
\begin{align*}
  \trgen{React}_q^D(\inp\chi_t(x).C) \is
    \nudge
    \set{\enctr{\q{send}, \s{\chi_t}{syn} D}
               {\q{rec},  \chi_t \s{C}{rec}}}
    \nudge\union
    \trgen{Spawn}(\q{rec}, q',\s{C}{rec},q, \nmig{C})
    \nudge\union
    \Union_{t' \in \Types} \trgen{Setup}(
      q', \qready,
      \s{\chi_{t'}}{msg}, \chi_{t'},
      \mig{C, t'}
    )
\end{align*}
where $q'$ is a fresh intermediate control state.
\egroup


==> definitions/setup.tex <==
Formally, suppose, for some $j$ and $k$,
  $\phi = \set{(x_1, \type_1)[\phi_1],\dots,(x_j, \type_j)[\phi_j]}
            \union
          \set{Q_1[],\dots,Q_k[]}$
where
  all $x_i$ are in $X_\Types$ and
  all $Q_i \in \Deriv$.
Then $\trgen{Setup}$ is defined as follows:
\bgroup
\newcommand{\nudge}{\\&\hspace{-4.5em}\union{}} %% Horrible spacing hack
% \newcommand{\nudge}{\\&{}\union{}}
% \newcommand{\nudge}{\\&\phantom{{}\is{}}}
\begin{align*}
  \trgen{Setup}(q,q',l,l',\phi)
    &  \is \set{\enctradd{q, l}{q_1, l}{\s{Q_1}{ready}}}
    \nudge \set{\enctradd{q_i,l}{q_{i+1},l}{\s{Q_{i+1}}{ready}} | 1 \leq i \leq j}
    \nudge \set{\enctradd{q_j,l}{q'_1,l}{\s{Q_j}{ready}}}
    \nudge \set{\enctradd{q'_i,l}{q''_i,l}{\s{x_i}{set}} | 1 \leq i \leq k}
    \nudge \Union_{i=1}^k \trgen{Setup}(q''_i,q'_{i+1},\s{x_i}{set},x_i,\phi_i)
    \nudge \set{\enctr{q'_{k+1},l}{q',l'}}
\end{align*}
where for all $1 \leq i \leq j$ and all $1 \leq i' \leq k$,
$q_i, q'_{i'}, q''_{i'}, q'_{k+1}$ are fresh intermediate control states.
in the sense that they are only mentioned in the transitions
generated by that specific application of $\trgen{Setup}$.
We allow $l$ to be the empty sequence,
in which case $l'$ needs to be the empty sequence as well.
\egroup

==> definitions/spawn.tex <==
Formally, let the forest $\phi = \Phi'(D)$ consist of trees $\lstc{\theta}{k}$,
for a term $D \in \Deriv$.
We can precompute, for each $\theta_i$, the base type
  $t_i \is \min_{\parent_\Types}\set{
    t | \chi_t \in \freenames(A), n \in N_{\theta_i}, \ell_{\theta_i}(n) = A}$
when defined.
For each label $\chi_t \in X_\Types$ we also have a label $\s{\chi_t}{sp}$
we write $\chi(\theta_i)$ (resp. $\s{\chi}{sp}(\theta_i)$)
for $\chi_{t_i}$ (resp. $\s{\chi_{t_i}}{sp}$) when $t_i$ is defined,
or the empty sequence when $t_i$ is undefined
(e.g.~when $\theta_i$ does not have free variables).
Then $\trgen{Spawn}(q,q',l,l',\phi)$ is the set of transition expressions
defined as follows:
\bgroup
\newcommand{\nudge}{\\&\hspace{-7.5em}} %% Horrible spacing hack
\begin{align*}
  \trgen{Spawn}(q_0,q',l,l',\phi)
    \is\nudge
    \set{\enctr{q_{i-1}, \chi(\theta_i)\:l}{q'_{i-1}, \s{\chi}{sp}(\theta_i)\:l}
          | 1 \leq i \leq k}
    \nudge\union{}
    \Union_{i=1}^k
      \trgen{Setup}(q'_{i-1}, q_i, \s{\chi}{sp}(\theta_i), \chi(\theta_i),\theta_i)
\end{align*}
where for all $1 < h \leq k$, $q_h, q'_h$ are fresh.
\egroup

==> definitions/statically-hierarchical.tex <==

\begin{definition}[Hierarchical term]
  A term $P\in\PiTerms$ is \emph{hierarchical}
  if there exist a finite forest $\Types$ and a $\Types$-annotated version $P^{\Types}$ of $P$ such that all terms reachable from $P^{\Types}$ are \tcompat.
\end{definition}


\begin{theorem}
  Determining whether an arbitrary \piterm{} is hierarchical, is decidable.
\end{theorem}

\newcommand{\BAD}{\mathit{Bad}_k^{\Types}}
\comment[ed]{%
  Lemma: Let $Q$ and $Q'$ be two terms such that $Q \embed Q'$.
         If $Q'$ is \tcompat\ then $Q$ is \tcompat\ as well.

  Proof of theorem:
    Let $k$ be the number of restrictions of $P$.
    If there exists a \Types\ proving $P$ hierarchical, there exists one with at most $k$ nodes.
    So we can restrict the check to the finitely many forests with $k$ nodes.

    First we can decide if $P$ is $k$-depth-bounded (decidability is proven in \cite{Huechting:14}).
    If it is not bounded in depth by $k$ then it is not hierarchical: there exists a reachable term where the forest needs to be higher than $k$.

    If $P$ is bounded in depth by $k$,
    for each choice of \Types\ we need to see if any term in the set
    \[
      \BAD \is \set{Q | \depth(Q) \leq k \land Q\text{ is not \tcompat}}
    \]
    is reachable.
    By Lemma above it suffices to check if any term in $\BAD$ is coverable from $P$.
    By wqo of term embedding for terms of depth bounded by $k$,
    we know that $\BAD$ has finitely many minimal elements $\set{Q_1, \dots, Q_m}$.
    Coverability is decidable since $P$ has been proven to be depth-bounded so we can check coverability of each $Q_i$.
    If any is coverable than we need to try with the next $\Types$, otherwise we have found a $\Types$ that proves $P$ hierarchical.
    If all the $\Types$ failed, than $P$ is not hierarchical.
}

While the property of being hierarchical is decidable, the algorithm that can be extracted from the decidability proof is extremely expensive computationally: it relies on solving many coverability problems over depth-bounded systems as sub-steps, each of which has non primitive recursive complexity.
In the next section we obviate to this problem by defining a type system
that is able to cheaply prove a term hierarchical with some mild approximation.


==> examples/repl-rule-extension.tex <==
Let
  $ A= \tact.\new b.\tact.\new c.\bang{(\out a<c> + \inp a(x).\out b<x>)} $
and consider the two terms
$P_1 = \new a.A$ and $P_2 = \new a.\bang{A}$.
The typing derivations for the two terms are almost identical and the set of constraints they impose on $\Types$ is the same.
However $P_1$ is depth bounded, $P_2$ is not.
Therefore the type system must reject both.
We briefly sketch a possible enhancement that is sensitive to replication.
Take the term
  $ \new b\tas t_b[t]. \new l\tas t_l[t]. \new r\tas t_r[t].
      \bang{\inp b(x).\inp l(y).(\out r<x> \parallel \out b<x>)} $
which acts as a 1 cell buffer between $l$ and $r$.
This term cannot be typed by the current type system because
  $\inp l(y).(\out r<x> \parallel \out b<x>)$
is migratable for the input $\inp b(x)$
thus requiring $t_l \tlt t_b$,
but at the same time $\out b<y>$ is migratable for $\inp l(y)$
requiring $t_b \tlt t_l$, leading to contradiction.
We propose to add to the structure of $\Types$ a notion of multiplicities
of base types; a base type can be marked with either $1$ or $\omega$.
Suppose the forest of a term has a path $p$ from a node $n$ to a node $n'$
where the trace of $p$ consists only of base types marked with $1$.
This situation will represent the fact that no branching will ever occur between the two replications corresponding to $n$ and $n'$ and having one of the two names in the scope guarantees that the other one is in the scope too.
In other words, all the restrictions represented by nodes in $p$ can be though as a indivisible unit;
when typing an input term on a name with base type $t$,
the constraints of rule~\ref{rule:in} can be relaxed to require the free variables of migratable terms to have base types smaller
than the lowest $t'$ such that the path between $t$ and $t'$ in $\Types$ is formed only of base types with multiplicity $1$.
In the case of buffer example, we observe that $b$, $l$ and $r$ could all be assigned base types of multiplicity $1$ thus replacing the two conflicting constraints with the constraints $t_l \leq t'$ and $t_b \leq t'$ where $t'$ is the greatest among $t_l$, $t_r$ and $t_b$.

==> proofs/encodingA.tex <==
By definition of $\AutEnc{P}$ we have $P \bisimA f_0$.
Showing that $\bisimA$ is indeed a bisimulation amounts to showing that
if $Q \bisimA f$ then:
\begin{enumerate}[label=(\Alph*)]
  \item for each $Q'$ such that $Q \redto Q'$
        there is a $f'$ such that $f \readyto f'$ and $Q' \bisimA f'$;
        \label{eq:bisim-proc}
  \item for each $f'$ such that $f \readyto f'$
        there is a $Q'$ such that $Q \redto Q'$ and $Q' \bisimA f'$.
        \label{eq:bisim-aut}
\end{enumerate}
To show this holds we rely on the hypothesis that $Q \bisimA f$
to get a $\iota$ relating $\Phi'(Q)$ and $f$.
The proof then closely follows the constructions
in the proof of Theorem~\ref{th:typed-tshaped}.
If $Q \redto Q'$ we can find two nodes $n_S$ and $n_R$ in $\Phi'(Q)$
labelled with the sender and receiver processes responsible for the reduction;
they will share an ancestor $n_a$ labelled $(\chi_t, t)$
corresponding to the channel on which they are synchronising.
On the automaton side, we have that $(\qready, f)$ matches the rule generated
from the sender by selecting the data value $d_S = \iota(n_S)$,
a data value $d_b$ corresponding to the name being sent and $d_a = \iota(n_a)$.
This leads to
$(q', f)$ where
  $f'(d_a) = \s{\chi_t}{syn}$,
  $f'(d_b) = \s{\chi_{t'}}{msg}$,
  $f'(d_S) = \s{S'}{wait}$.
From here only one of the transitions generated from $\trgen{Spawn}$
of the continuation is enabled as there is only one node marked with `wait'.
The transitions are deterministic from here until a configuration
$(\q{send}, f')$ is reached with $f'$ representing the initial forest with
the continuation of the sender added and with the node of the sender updated
with either $\qdead$ or the sender itself if it is a replicated component.
At this point there is only one data value marked with `syn' and
the only transitions from $\q{send}$ are the ones generated from a process
that can receive from the marked channel.
We can pick the rule that has been generated
from the receiver involved in the reduction from $Q$ to $Q'$
and go to a configuration with control state $\q{rec}$.
From this configuration the transitions are deterministic.
The next configuration reached with control state
$\qready$ is bisimilar to $Q'$ by tracing the effects these transitions have
on the class memory function.
Fresh data values get assigned labels compatible with the non migrating
continuations of the receiver first,
and then the migrating ones as children of $d_b$;
data values with meaningless labels get assigned the label $\qdead$.

To prove~\ref{eq:bisim-aut} we proceed similarly.
Every reduction sequence from $(\qready, f)$ to $(\qready, f')$
must start with a transition to a configuration with control state $\q{send}$,
which is generated by rules extracted from a sender $S$
labelling a data value $d_S$;
since $Q \bisimA f$ we know that $n_S = \inv\iota(d_S)$ is labelled with $S$
in $\Phi'(Q)$, hence $S$ is an active sequential process of $Q$.
To complete this part of the proof we only need to follow the transitions
of the automaton in the same way as done for the previous point,
and note that the only way the automaton can reach a configuration
with control state $\qready$ from $(\qready, f)$
is by selecting a receiver that can synchronise with the selected sender.
This is important because there may be transitions from $(\qready, f)$
corresponding to selecting a sender trying to synchronise
on a channel on which no receiver is listening.
This transition would lead to a deadlocked configuration
(one with no successors)
but never going through a configuration with control state $\qready$.


==> proofs/encodingP-hierarchical.tex <==
Assume an arbitrary strict total order $<_\States$
on the automaton's control states;
let then $(\Types, \parent)$ be the forest with nodes
  $\Types = \set{t_{c^i_q} | 0 \leq i \leq \ell, q \in \States}$
and $t_{c^i_q} \parent t_{c^i_{q'}}$ if $q <_\States q'$,
and $t_{c^i_q} \parent t_{c^{i+1}_{q'}}$ if $q$ and $q'$ are respectively
the maximum and minimum states with respect to $<_\States$.
It can be proved that $\emptyset \types \nf(\ProcEnc{\Aut})$:
since no messages are exchanged over channels, the constraints on types
are trivially satisfied;
for the same reason, no sequential term under an input prefix is migratable,
making all the base type constraints in rule~\ref{rule:in} trivially valid.
The base type inequalities of rule~\ref{rule:conf} are also satisfied since
in $A_\tr$ for $\tr \in \theta_j$, every $P_{\theta_k}$ might be tied to any channel $c$ in $\Chan^{j+1}\union\dots\union\Chan^{i}$
but can only have as free names channels in $\Chan^h$ with $h \leq j$,
which all have base types smaller than $c$.

==> proofs/encodingP.tex <==
Fix an \NDA\ $\Aut = (\States, \delta, q_0, f_0)$
with $\delta = \Union_{0 \leq j \leq \ell} \theta_j$ as before.
We prove the theorem by exhibiting a bisimulation relation
$(\bisimP) \subseteq
  (\States \times (\dataset \pto \States_\fresh)) \times \reach(\ProcEnc{\Aut})$
between the two transition systems.
For a class memory function $f \from \dataset \to \States_\fresh$,
let $f(\dataset)$ be the $\States$-labelled forest with
the set $N=\set{ d \in \dataset | f(d) \neq \fresh }$ as nodes,
each labelled with $f(d)$
and with $\pred_\dataset$ restricted to $N$ as parent relation.
We first define a hierarchy of relations $\bisimP_i$
between $\States$-labelled forests and \piterm{s},
for $0 \leq i \leq \ell$, as follows:
$
  q[\set{\lstc{\phi}{n}}]
    \bisimP_i
  \new \Chan^i.(
    P_{\theta_i} \parallel
    \outz c^i_q \parallel
    \Parallel_{1 \leq j \leq n} P_j
  )
$
if, for all $1 \leq j \leq n$, $\phi_j \bisimP_{i+1} P_j$.
Since $n$ must be 0 for $i=\ell$, the relation is well-defined.
Let $P \in \reach(\ProcEnc{\Aut})$ and $(q, f)$ be a reachable configuration of \Aut.
Then $(q, f) \bisimP P$ if there exists a $P' \congr P$ such that
$q_0[f(\dataset)] \bisimP_0 P'$.
To show that $\bisimP$ is indeed a bisimulation, we have to prove that
if $(q,f) \bisimP P$ then:
\begin{enumerate}[label=(\Alph*)]
  \item for each $(q',f')$ such that $(q,f) \autto (q',f')$
        there is a $P'$ such that $P \chanzto P'$ and $(q',f') \bisimP P'$;
        \label{eq:bisim-bis-aut}
  \item for each $P'$ such that $P \chanzto P'$
        there is a $(q',f')$ such that $(q,f) \autto (q',f')$
        and $P' \bisimP (q',f')$.
        \label{eq:bisim-bis-proc}
\end{enumerate}
To prove \ref{eq:bisim-bis-aut} we proceed as follows;
suppose $(q,f) \autto (q',f')$ is an application of a transition
$t = (q, \lst[1]{q}{j}, \fresh,\dots,\fresh,
  q', \lst[1]{q'}{i}) \in \theta_j$
then the forest $q[f(\dataset)]$ has a path from the root to a leaf
labelled with $q,\lstc{q}{j}$, which, by definition of $\bisimP$,
implies that $P$ is congruent to a term with the following shape:
\[
  \new \Chan^0.(
    R_0 \parallel
    \outz c^0_q \parallel
    \new \Chan^1.(
      R_1 \parallel
      \outz c^1_{q_1} \parallel
      \cdots
        \new \Chan^j.(
          R_j \parallel
          \outz c^j_{q_j} \parallel
          P_{\theta_j}
        )
      \cdots
    ).
\]
By construction, $P_{\theta_j} \congr \bang{(A_\tr)} \parallel R$ and
$A_\tr$ is a process inputting once from $c^0_q$ then
once from each $c^k_{q_k}$ in sequence.
From the shape of $P$ we can conclude all of these input prefixes
can synchronise with the dual $\outz c^k_{q_k}$ processes
in parallel with them, activating, in $j+1$ steps, the continuation
$C =
  \new \Chan^{j+1}. \cdots \new \Chan^{i}.
    \left(
    \outz c^0_{q'} \parallel
    \Parallel_{k=1}^\ell \outz c^k_{q'_k}
      \parallel
    P_{\theta_{j+1}}
    \right)$,
yielding the process
\[
  P' \congr \new \Chan^0.(
    R_0 \parallel
    \outz c^0_{q'} \parallel
    \new \Chan^1.(
      R_1 \parallel
      \outz c^1_{q'_1} \parallel
      \cdots
        \new \Chan^i.(
          R_i \parallel
          \outz c^j_{q'_j}
        )
      \cdots
    )
\]
where for $k$ between $j+1$ and $i$, $R_k = P_{\theta_k}$.
Now consider the forest $q'[f'(\dataset)]$:
it coincides with $q[f(\dataset)]$ except
on the path we singled out, now labelled with
$q', q'_0, \dots, q'_j$ and continuing to a leaf
with nodes labelled $q'_{j+1},\dots,q'_i$.
It is easy to see that $q'[f'(\dataset)] \bisimP P'$.

To prove \ref{eq:bisim-bis-proc} one can proceed similarly,
by observing that even if $\ProcEnc{\Aut}$ can perform some reductions which deadlock
that do not correspond to reductions of the automaton,
these steps cannot lead to a state with $\outz c^0_{q'}$
as one of the active sequential processes.
This claim is supported by the following easy to verify invariant:
in any term $P$ reachable from $\ProcEnc{\Aut}$, for each bound name $c$ in $P$
there is at most one active sequential subterm of $P$ outputting on $c$.
This is satisfied by $\ProcEnc{\Aut}$ and preserved by reduction.


==> proofs/forest-nf-sketch.tex <==
By induction on the structure of $\phi$.


==> proofs/subj-red-sketch.tex <==
From $P\redto Q$ we know that
$P \congr \new W.(S \parallel R \parallel C)$,
$S \congr \out a<b>.\new Y_s.(S'+M_s)$,
$R \congr \inp a(x).\new Y_r.(R'+M_r)$,
$Q \congr \new W Y'_s Y'_r.
  (S'\sigma_s \parallel R'\subst{x->b}\:\sigma_r \parallel C)$
where $\sigma_k \is \subst{y->y'}_{y\in Y_k}$,
and $Y'_k \is \Set{y'|y\in Y_k}$ are fresh names,
for $k\in\set{s,r}$.
Then it is easy to verify that
the typing proof of $P$ can be easily adapted to be one for $Q$;
the non trivial step is showing that
the premises involving $R'\subst{x->b}$ are true;
for this we can use Lemma~\ref{lemma:subst}.


==> proofs/typed-tshaped-sketch.tex <==
The full proof is presented in~\appendixorfull.
We outline here only the crucial steps.
Consider the input output synchronisation case where the sending action $\out a<b>$ is such that
$\restr (a \tas \type_a)$ and $\restr (b \tas \type_b)$ are both active restrictions of $P$ and $t_a=\base(\type_a)\tlt\base(\type_b)=t_b$.
As in the proof of Theorem~\ref{th:subj-red}, the derivation of $\Env \types P$
must follow the shape of \eqref{eq:P-deriv}.
From \tshaped[ness] of $P$ we can conclude that
both $\new Y_s.S'$ and $\new Y_r.R'$ are \tshaped.
By Lemma~\ref{lemma:phi-tcompat} we know that
  $\phi   = \Phi(\new W.(S \parallel R \parallel C)) \in \AST{P}$,
  $\phi_r = \Phi(\new Y_r.R'\subst{a->b}) \in \AST{\new Y_r.R'\subst{x->b}}$ and
  $\phi_s = \Phi(\new Y_s.S') \in \AST{\new Y_s.S'}$.
Let $\phi_r = \phimig \dunion \phinonmig$
where only $\phimig$ contains a leaf labelled with a term with $b$ as a free name.
These leaves will correspond to the continuations $R'_j$
that migrate in $\inp a(x).\new Y_r.R'$,
after the application of the substitution $\subst{x->b}$.
By assumption, inside $P$ both $S$ and $R$ are in the scope of the restriction bounding $a$
and $S$ must also be in the scope of the restriction bounding $b$.
% Let $t_a = \base(\type_a)$ and $t_b = \base(\type_b)$,
$\phi$ will contain two leaves $n_S$ and $n_R$
labelled with $S$ and $R$ respectively,
having a common ancestor $n_a$ labelled with $(a, t_a)$;
$n_S$ will have an ancestor $n_b$ labelled with $(b, t_b)$.
Let $p_a$, $p_S$ and $p_R$ be the paths in $\phi$ leading from a root to $n_a$, $n_S$ and $n_R$ respectively.
\newcommand{\parentins}{\parent_{\mathrm{ins}}}
Now, we want to transform $\phi$, by manipulating this tree,
into a forest $\phi'$ that is
\tcompat\ by construction and such that
there exists a term $Q' \congr Q$ with $\forest(Q') = \phi'$,
so that we can conclude $Q$ is \tshaped.

To do so, we introduce the following function,
taking a labelled forest $\phi$, a path $p$ in $\phi$ and a labelled forest $\rho$
and returning a labelled forest:
$  \treeins(\phi, p, \rho) \is (
    N_\phi \dunion N_\rho,
    \parent_\phi \dunion \parent_\rho \dunion \parentins,
    \ell_\phi \dunion \ell_\rho
  )$
where $n\parentins n'$ if
  $n' \in \min_{\parent_\rho}(N_\rho)$
and if $\ell_\rho(n') = (y, t_y)$ then
$
  n \in \max_{\parent_\phi}\set{m \in p | \ell_\phi(m) = (x,t_x), t_x < t_y}
$
or if $\ell_\rho(n') = A$ then
$
  n \in \max_{\parent_\phi}\set{m \in p | \ell_\phi(m) = (x,t_x), x \in \freenames(A)}
$.
Note that for each $n'$, since $p$ is a path, there can be at most one $n$ such that $n \parentins n'$.
To obtain the desired $\phi'$,
we first need to remove the leaves $n_S$ and $n_R$ from $\phi$,
as they represent the sequential processes which reacted,
obtaining a forest $\phi_C$.
We argue that the $\phi'$ we need is indeed
  $\phi' = \treeins(\phi_1, p_S, \phimig)$ where
  $\phi_1 = \treeins(\phi_2, p_R, \phinonmig)$ and
  $\phi_2 = \treeins(\phi_C, p_S, \phi_s)$.
It is easy to see that, by definition of $\treeins$, $\phi'$ is \tcompat:
$\phi_C$, $\phi_s$, $\phinonmig$ and $\phimig$ are \tcompat\ by hypothesis,
$\treeins$ adds parent-edges only when they do not break \tcompat[ibility].

The proof is completed by showing that $\phi'$ is the forest of a term congruent to
  $\new W Y_s Y_r.(S' \parallel R'\subst{x->b} \parallel C)$
using Lemma~\ref{lemma:forest-nf}.


==> style/comments.tex <==
\usepackage[nosign]{commenting}

\declareauthor{ed}{Manu}{green!50!black}
\authorcommand{ed}{comment}
\declareauthor{lo}{Luke}{red}
\authorcommand{lo}{comment}
\setdefaultauthor{ed}

\makeatletter
\renewcommand{\comm@todo@mpar}[1]{}
\makeatother

\def\divider{%
  \leavevmode\leaders\hrule height 0.6ex depth \dimexpr0.4pt-0.6ex\hfill%
  \kern0pt%
}
\newcommand{\ONGOING}[1]{%
  \draftpar\comment*{\divider\MakeUppercase{Ongoing~#1}\divider}\draftpar%
}

\renewcommand{\OpenCommentBraket}{$\lceil$}
\renewcommand{\ClosedCommentBraket}{$\rfloor$}


==> style/layout.tex <==
\usepackage{fixltx2e}
\usepackage[inline]{enumitem}
\setlist[itemize]{label=-}

\newlist{defenum}{enumerate}{2}
\setlist[defenum]{
  label=\small(\roman*),
  % ref=\thedefinition.\roman*,
  % labelwidth=3pt,
  leftmargin=2em
}

\newlist{asparaenum}{enumerate}{3}
\setlist[asparaenum]{label=(\roman*), align=left, leftmargin=0pt, labelindent=!, listparindent=\parindent, labelwidth=0pt, itemindent=!}

\newlist{inparaenum}{enumerate*}{3}
\setlist[inparaenum]{label=\alph*)}

\newlist{asparaitem}{enumerate}{3}
\setlist[asparaitem]{label=-, align=left, leftmargin=0pt, labelindent=!, listparindent=\parindent, labelwidth=0pt, itemindent=!}

% \usepackage{booktabs}
% \usepackage{multirow}

\RequirePackage{xcolor}
\RequirePackage{hyperref}
\hypersetup{final}
\hypersetup{%
    % bookmarks,
    bookmarksopen,
    % bookmarksnumbered,
    colorlinks,
    linkcolor=blue,
    citecolor=brown,
    % backref,
    urlcolor=blue,
    pdfstartview=FitH}
% \urlstyle{same}  % don't use monospace font for urls

\makeatletter
% \@beginparpenalty=10000
\def\donotbreak{\@beginparpenalty=10000}

\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                       {-12\p@ \@plus -4\p@ \@minus -4\p@}%
                       {-0.5em \@plus -0.22em \@minus -0.1em}%
                       {\normalfont\normalsize\bfseries\boldmath}}

\newenvironment{trickspacing}{%
  \def\@Thm##1##2##3{\topsep 5\p@ \@plus2\p@ \@minus4\p@%
  \@ifnextchar[{\@Ythm{##1}{##2}{##3}}{\@Xthm{##1}{##2}{##3}}}%
}{}

\g@addto@macro{\appendix}{%
  \thispagestyle{empty}%
  \phantomsection%
  \label{appendix}%
  \pdfbookmark{Appendix}{appendix-b}%
  \centerline{\Large\textbf{Appendix}}\bigskip%
}

\makeatother

\let\import\input

\usepackage[caption=false]{subfig}


==> style/no-tikz.tex <==
\usepackage{graphicx}
\def\tikzset#1{}%
\def\tikzsetnextfilename#1{}%
\newcommand{\ExportTikzPictures}{}
\def\inputfig#1{\IfFileExists{export/#1.patch.tex}{\input{export/#1.patch.tex}}{}\includegraphics{export/#1}}
\newcommand{\inputfigwrap}[2][]{\inputfig{#2}}
\newenvironment{tikzpicture}[1][]{}{}
